On denoising modulo 1 samples of a function

Consider an unknown smooth function $f: [0,1] \rightarrow \mathbb{R}$, and say we are given $n$ noisy$\mod 1$ samples of $f$, i.e., $y_i = (f(x_i) + \eta_i)\mod 1$ for $x_i \in [0,1]$, where $\eta_i$ denotes noise. Given the samples $(x_i,y_i)_{i=1}^{n}$ our goal is to recover smooth, robust estimates of the clean samples $f(x_i) \bmod 1$. We formulate a natural approach for solving this problem which works with representations of mod 1 values over the unit circle. This amounts to solving a quadratically constrained quadratic program (QCQP) with non-convex constraints involving points lying on the unit circle. Our proposed approach is based on solving its relaxation which is a trust-region sub-problem, and hence solvable efficiently. We demonstrate its robustness to noise % of our approach via extensive simulations on several synthetic examples, and provide a detailed theoretical analysis.

==> AISTATS_figures_ScanID_1.tex <==

\begin{figure*}
\centering
\subcaptionbox[]{ $k=2$, $\lambda= 0.03$
% \label{subfig:sublabel3}
}[ 0.24\textwidth ]
{\includegraphics[width=0.24\textwidth] {figs/PLOTS_SCANS/f1_Bounded_scanID_1_nrR_20/f1_Bounded_fmod1_n_500_k_2_lambda_0p03_scanID_1_nrReps_20.eps} }
% \hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{ $k=3$, $\lambda= 0.03$
% \label{subfig:sublabel3}
}[ 0.24\textwidth ]
{\includegraphics[width=0.24\textwidth] {figs/PLOTS_SCANS/f1_Bounded_scanID_1_nrR_20/f1_Bounded_fmod1_n_500_k_3_lambda_0p03_scanID_1_nrReps_20.eps} }
% \hspace{0.01\textwidth} % seperation
%
%------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------
%
\subcaptionbox[]{ $k=2$, $\lambda= 0.3$
% \label{subfig:sublabel3}
}[ 0.24\textwidth ]
{\includegraphics[width=0.24\textwidth] {figs/PLOTS_SCANS/f1_Bounded_scanID_1_nrR_20/f1_Bounded_fmod1_n_500_k_2_lambda_0p3_scanID_1_nrReps_20.eps} }
% \hspace{0.01\textwidth} % seperation
%------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------
%
\subcaptionbox[]{ $k=2$, $\lambda= 0.5$
% \label{subfig:sublabel3}
}[ 0.24\textwidth ]
{\includegraphics[width=0.24\textwidth] {figs/PLOTS_SCANS/f1_Bounded_scanID_1_nrR_20/f1_Bounded_fmod1_n_500_k_2_lambda_0p5_scanID_1_nrReps_20.eps} }
% \hspace{0.01\textwidth} % seperation
%
%------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------
\vspace{3mm}
\caption[Short Caption]{ f1 Bounded: f mod 1, nrReps = 20, scanID = 1 
% Numerical results for the function XYZ, under the Gaussian noise model.  Results are averaged over 20 trials, $n=500, k \in  \{ 2,3,5 \}$ and $\lambda \in \{ 0.1, 0.3, 0.5, 1 \} $  
}
\label{fig:Sims_f1_Bounded_fmod1}
\end{figure*}

 



\begin{figure*}
\centering
\subcaptionbox[]{ $k=2$, $\lambda= 0.03$
% \label{subfig:sublabel3}
}[ 0.24\textwidth ]
{\includegraphics[width=0.24\textwidth] {figs/PLOTS_SCANS/f1_Bounded_scanID_1_nrR_20/f1_Bounded_f_n_500_k_2_lambda_0p03_scanID_1_nrReps_20.eps} }
% \hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{ $k=3$, $\lambda= 0.03$
% \label{subfig:sublabel3}
}[ 0.24\textwidth ]
{\includegraphics[width=0.24\textwidth] {figs/PLOTS_SCANS/f1_Bounded_scanID_1_nrR_20/f1_Bounded_f_n_500_k_3_lambda_0p03_scanID_1_nrReps_20.eps} }
\hspace{0.01\textwidth} % seperation
%
%------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------
%
\subcaptionbox[]{ $k=2$, $\lambda= 0.3$
% \label{subfig:sublabel3}
}[ 0.24\textwidth ]
{\includegraphics[width=0.24\textwidth] {figs/PLOTS_SCANS/f1_Bounded_scanID_1_nrR_20/f1_Bounded_f_n_500_k_2_lambda_0p3_scanID_1_nrReps_20.eps} }
% \hspace{0.01\textwidth} % seperation
%
%------------------------------------------------------------------------------------------
\subcaptionbox[]{ $k=2$, $\lambda= 0.5$
% \label{subfig:sublabel3}
}[ 0.24\textwidth ]
{\includegraphics[width=0.24\textwidth] {figs/PLOTS_SCANS/f1_Bounded_scanID_1_nrR_20/f1_Bounded_f_n_500_k_2_lambda_0p5_scanID_1_nrReps_20.eps} }
% \hspace{0.01\textwidth} % seperation
%
%------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------
\vspace{3mm}
\caption[Short Caption]{ f1 Bounded: f, nrReps = 20, scanID = 1 
% Numerical results for the function XYZ, under the Gaussian noise model.  Results are averaged over 20 trials, $n=500, k \in  \{ 2,3,5 \}$ and $\lambda \in \{ 0.1, 0.3, 0.5, 1 \} $  
}
\label{fig:Sims_f1_Bounded_f}
\end{figure*}




\begin{figure*}
\centering
\subcaptionbox[]{ $k=2$, $\lambda= 0.1$
% \label{subfig:sublabel3}
}[ 0.24\textwidth ]
{\includegraphics[width=0.24\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_1_nrR_20/f1_Gaussian_fmod1_n_500_k_2_lambda_0p1_scanID_1_nrReps_20.eps} }
%\hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{ $k=3$, $\lambda= 0.1$
% \label{subfig:sublabel3}
}[ 0.24\textwidth ]
{\includegraphics[width=0.24\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_1_nrR_20/f1_Gaussian_fmod1_n_500_k_3_lambda_0p1_scanID_1_nrReps_20.eps} }
% \hspace{0.01\textwidth} % seperation
%------------------------------------------------------------------------------------------
%
\subcaptionbox[]{ $k=2$, $\lambda= 0.3$
% \label{subfig:sublabel3}
}[ 0.24\textwidth ]
{\includegraphics[width=0.24\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_1_nrR_20/f1_Gaussian_fmod1_n_500_k_2_lambda_0p3_scanID_1_nrReps_20.eps} }
%\hspace{0.01\textwidth} % seperation
%------------------------------------------------------------------------------------------
%
\subcaptionbox[]{$k=2$, $\lambda= 0.5$
% \label{subfig:sublabel3}
}[ 0.24\textwidth]
{\includegraphics[width=0.24\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_1_nrR_20/f1_Gaussian_fmod1_n_500_k_2_lambda_0p5_scanID_1_nrReps_20.eps} }
%\hspace{0.01\textwidth} % seperation
%------------------------------------------------------------------------------------------
\vspace{3mm}
\caption[Short Caption]{ f1 Gaussian: f mod 1, nrReps = 20, scanID = 1 
% Numerical results for the function XYZ, under the Gaussian noise model.  Results are averaged over 20 trials, $n=500, k \in  \{ 2,3,5 \}$ and $\lambda \in \{ 0.1, 0.3, 0.5, 1 \} $  
}
\label{fig:Sims_f1_Gaussian_fmod1}
\end{figure*}

 



\begin{figure*}
\centering
\subcaptionbox[]{ $k=2$, $\lambda= 0.1$
% \label{subfig:sublabel3}
}[ 0.24\textwidth ]
{\includegraphics[width=0.24\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_1_nrR_20/f1_Gaussian_f_n_500_k_2_lambda_0p1_scanID_1_nrReps_20.eps} }
%\hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{ $k=3$, $\lambda= 0.1$
% \label{subfig:sublabel3}
}[ 0.24\textwidth ]
{\includegraphics[width=0.24\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_1_nrR_20/f1_Gaussian_f_n_500_k_3_lambda_0p1_scanID_1_nrReps_20.eps} }
%\hspace{0.01\textwidth} % seperation
%------------------------------------------------------------------------------------------
\subcaptionbox[]{ $k=2$, $\lambda= 0.3$
% \label{subfig:sublabel3}
}[ 0.24\textwidth ]
{\includegraphics[width=0.24\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_1_nrR_20/f1_Gaussian_f_n_500_k_2_lambda_0p3_scanID_1_nrReps_20.eps} }
% \hspace{0.01\textwidth} % seperation
%------------------------------------------------------------------------------------------
\subcaptionbox[]{ $k=2$, $\lambda= 0.5$
% \label{subfig:sublabel3}
}[ 0.24\textwidth ]
{\includegraphics[width=0.24\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_1_nrR_20/f1_Gaussian_f_n_500_k_2_lambda_0p5_scanID_1_nrReps_20.eps} }
% \hspace{0.01\textwidth} % seperation
%------------------------------------------------------------------------------------------
\vspace{3mm}
\caption[Short Caption]{ f1 Gaussian: f, nrReps = 20, scanID = 1 
% Numerical results for the function XYZ, under the Gaussian noise model.  Results are averaged over 20 trials, $n=500, k \in  \{ 2,3,5 \}$ and $\lambda \in \{ 0.1, 0.3, 0.5, 1 \} $  
}
\label{fig:Sims_f1_Gaussian_f}
\end{figure*}


==> AISTATS_figures_ScanID_2.tex <==

 
Figure \ref{fig:Sims_f1_Bounded_ScanID2_fmod1}, respectively Figure \ref{fig:Sims_f1_Bounded_ScanID2_f}, show the RMSE (on a log scale) for the $f \mod 1$ denoising, respectively the recovery of the full function $f$, as we increase the number of samples  $n$, for a fixed value of $\lambda=0.3$, and $k=\{ 2,3 \}$,  as we vary the noise level $\gamma = \{0.01, 0.25\}$ under the Uniform noise model.


\begin{figure}
\centering
%%%%
\subcaptionbox[]{ $k=2$, $\lambda= 0.3$, $\gamma = 0.01$
% \label{subfig:sublabel3}
}[ 0.22\textwidth ]
{\includegraphics[width=0.22\textwidth] {figs/PLOTS_SCANS/f1_Bounded_scanID_2_nrR_10/f1_Bounded_fmod1_sigma_0p01_k_2_lambda_0p3_scanID_2_nrReps_10.eps} }
\hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{ $k=3$, $\lambda= 0.3$, $\gamma = 0.25$
% \label{subfig:sublabel3}
}[ 0.22\textwidth ]
{\includegraphics[width=0.22\textwidth] {figs/PLOTS_SCANS/f1_Bounded_scanID_2_nrR_10/f1_Bounded_fmod1_sigma_0p25_k_3_lambda_0p3_scanID_2_nrReps_10.eps} }
\hspace{0.01\textwidth} % seperation
%------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------
\vspace{3mm}
\caption[Short Caption]{ f1 Bounded: f mod 1, nrReps = 10, scanID = 2
% Numerical results for the function XYZ, under the Gaussian noise model.  Results are averaged over 20 trials, $n=500, k \in  \{ 2,3,5 \}$ and $\lambda \in \{ 0.1, 0.3, 0.5, 1 \} $  
}
\label{fig:Sims_f1_Bounded_ScanID2_fmod1}
\end{figure}


\begin{figure}
\centering
\subcaptionbox[]{ $k=2$, $\lambda= 0.3$, $\delta = 0.01$
% \label{subfig:sublabel3}
}[ 0.22\textwidth ]
{\includegraphics[width=0.22\textwidth] {figs/PLOTS_SCANS/f1_Bounded_scanID_2_nrR_10/f1_Bounded_f_sigma_0p01_k_2_lambda_0p3_scanID_2_nrReps_10.eps} }
\hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{ $k=3$, $\lambda= 0.3$, $\delta = 0.25$
% \label{subfig:sublabel3}
}[ 0.22\textwidth ]
{\includegraphics[width=0.22\textwidth] {figs/PLOTS_SCANS/f1_Bounded_scanID_2_nrR_10/f1_Bounded_f_sigma_0p25_k_3_lambda_0p3_scanID_2_nrReps_10.eps} }
\hspace{0.01\textwidth} % sepe, ration
%------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------
\vspace{3mm}
\caption[Short Caption]{Recovery errors under the Uniform noise model, for different values of $k$, $\lambda$ and $\delta$. Results averaged over 10 runs.
% f1 Bounded: f, nrReps = 10, scanID = 2
% Numerical results for the function XYZ, under the Gaussian noise model.  Results are averaged over 20 trials, $n=500, k \in  \{ 2,3,5 \}$ and $\lambda \in \{ 0.1, 0.3, 0.5, 1 \} $  
}
\label{fig:Sims_f1_Bounded_ScanID2_f}
\end{figure}




%
%
%
%
%

\iffalse

\begin{figure*}
\centering
%%%%
\subcaptionbox[]{ $k=2$, $\lambda= 0.1$, $\sigma = 0.01$
% \label{subfig:sublabel3}
}[ 0.231\textwidth ]
{\includegraphics[width=0.23\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_2_nrR_10/f1_Gaussian_fmod1_sigma_0p01_k_2_lambda_0p1_scanID_2_nrReps_10.eps} }
\hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{ $k=3$, $\lambda= 0.1$, $\sigma = 0.01$
% \label{subfig:sublabel3}
}[ 0.231\textwidth ]
{\includegraphics[width=0.23\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_2_nrR_10/f1_Gaussian_fmod1_sigma_0p01_k_3_lambda_0p1_scanID_2_nrReps_10.eps} }
\hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{ $k=2$, $\lambda= 0.3$, $\sigma = 0.01$
% \label{subfig:sublabel3}
}[ 0.231\textwidth ]
{\includegraphics[width=0.23\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_2_nrR_10/f1_Gaussian_fmod1_sigma_0p01_k_2_lambda_0p3_scanID_2_nrReps_10.eps} }
\hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{ $k=3$, $\lambda= 0.3$, $\sigma = 0.01$
% \label{subfig:sublabel3}
}[ 0.231\textwidth ]
{\includegraphics[width=0.23\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_2_nrR_10/f1_Gaussian_fmod1_sigma_0p01_k_3_lambda_0p3_scanID_2_nrReps_10.eps} }
\hspace{0.01\textwidth} % seperation
%------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------
%
%
%
\subcaptionbox[]{ $k=2$, $\lambda= 0.1$, $\sigma = 0.05$
% \label{subfig:sublabel3}
}[ 0.231\textwidth ]
{\includegraphics[width=0.23\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_2_nrR_10/f1_Gaussian_fmod1_sigma_0p05_k_2_lambda_0p1_scanID_2_nrReps_10.eps} }
\hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{ $k=3$, $\lambda= 0.1$, $\sigma = 0.05$
% \label{subfig:sublabel3}
}[ 0.231\textwidth ]
{\includegraphics[width=0.23\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_2_nrR_10/f1_Gaussian_fmod1_sigma_0p05_k_3_lambda_0p1_scanID_2_nrReps_10.eps} }
\hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{ $k=2$, $\lambda= 0.3$, $\sigma = 0.05$
% \label{subfig:sublabel3}
}[ 0.231\textwidth ]
{\includegraphics[width=0.23\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_2_nrR_10/f1_Gaussian_fmod1_sigma_0p05_k_2_lambda_0p3_scanID_2_nrReps_10.eps} }
\hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{ $k=3$, $\lambda= 0.3$, $\sigma = 0.05$
% \label{subfig:sublabel3}
}[ 0.231\textwidth ]
{\includegraphics[width=0.23\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_2_nrR_10/f1_Gaussian_fmod1_sigma_0p05_k_3_lambda_0p3_scanID_2_nrReps_10.eps} }
\hspace{0.01\textwidth} % seperation
%------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------
%
%
%
%
%
\subcaptionbox[]{ $k=2$, $\lambda= 0.1$, $\sigma = 0.15$
% \label{subfig:sublabel3}
}[ 0.231\textwidth ]
{\includegraphics[width=0.23\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_2_nrR_10/f1_Gaussian_fmod1_sigma_0p15_k_2_lambda_0p1_scanID_2_nrReps_10.eps} }
\hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{ $k=3$, $\lambda= 0.1$, $\sigma = 0.15$
% \label{subfig:sublabel3}
}[ 0.231\textwidth ]
{\includegraphics[width=0.23\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_2_nrR_10/f1_Gaussian_fmod1_sigma_0p15_k_3_lambda_0p1_scanID_2_nrReps_10.eps} }
\hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{ $k=2$, $\lambda= 0.3$, $\sigma = 0.15$
% \label{subfig:sublabel3}
}[ 0.231\textwidth ]
{\includegraphics[width=0.23\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_2_nrR_10/f1_Gaussian_fmod1_sigma_0p15_k_2_lambda_0p3_scanID_2_nrReps_10.eps} }
\hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{ $k=3$, $\lambda= 0.3$, $\sigma = 0.15$
% \label{subfig:sublabel3}
}[ 0.231\textwidth ]
{\includegraphics[width=0.23\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_2_nrR_10/f1_Gaussian_fmod1_sigma_0p15_k_3_lambda_0p3_scanID_2_nrReps_10.eps} }
\hspace{0.01\textwidth} % seperation
%------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------
%
%%%%%%
\subcaptionbox[]{ $k=2$, $\lambda= 0.1$, $\sigma = 0.25$
% \label{subfig:sublabel3}
}[ 0.231\textwidth ]
{\includegraphics[width=0.23\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_2_nrR_10/f1_Gaussian_fmod1_sigma_0p25_k_2_lambda_0p1_scanID_2_nrReps_10.eps} }
\hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{ $k=3$, $\lambda= 0.1$, $\sigma = 0.25$
% \label{subfig:sublabel3}
}[ 0.231\textwidth ]
{\includegraphics[width=0.23\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_2_nrR_10/f1_Gaussian_fmod1_sigma_0p25_k_3_lambda_0p1_scanID_2_nrReps_10.eps} }
\hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{ $k=2$, $\lambda= 0.3$, $\sigma = 0.25$
% \label{subfig:sublabel3}
}[ 0.231\textwidth ]
{\includegraphics[width=0.23\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_2_nrR_10/f1_Gaussian_fmod1_sigma_0p25_k_2_lambda_0p3_scanID_2_nrReps_10.eps} }
\hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{ $k=3$, $\lambda= 0.3$, $\sigma = 0.25$
% \label{subfig:sublabel3}
}[ 0.231\textwidth ]
{\includegraphics[width=0.23\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_2_nrR_10/f1_Gaussian_fmod1_sigma_0p25_k_3_lambda_0p3_scanID_2_nrReps_10.eps} }
\hspace{0.01\textwidth} % seperation
%------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------
\vspace{3mm}
\caption[Short Caption]{ f1 Gaussian: f mod 1, nrReps = 10, scanID = 2
% Numerical results for the function XYZ, under the Gaussian noise model.  Results are averaged over 20 trials, $n=500, k \in  \{ 2,3,5 \}$ and $\lambda \in \{ 0.1, 0.3, 0.5, 1 \} $  
}
\label{fig:Sims_f1_Gaussian_ScanID2_fmod1}
\end{figure*}


\begin{figure*}
\centering
%%%%
\subcaptionbox[]{ $k=2$, $\lambda= 0.1$, $\sigma = 0.01$
% \label{subfig:sublabel3}
}[ 0.231\textwidth ]
{\includegraphics[width=0.23\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_2_nrR_10/f1_Gaussian_f_sigma_0p01_k_2_lambda_0p1_scanID_2_nrReps_10.eps} }
\hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{ $k=3$, $\lambda= 0.1$, $\sigma = 0.01$
% \label{subfig:sublabel3}
}[ 0.231\textwidth ]
{\includegraphics[width=0.23\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_2_nrR_10/f1_Gaussian_f_sigma_0p01_k_3_lambda_0p1_scanID_2_nrReps_10.eps} }
\hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{ $k=2$, $\lambda= 0.3$, $\sigma = 0.01$
% \label{subfig:sublabel3}
}[ 0.231\textwidth ]
{\includegraphics[width=0.23\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_2_nrR_10/f1_Gaussian_f_sigma_0p01_k_2_lambda_0p3_scanID_2_nrReps_10.eps} }
\hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{ $k=3$, $\lambda= 0.3$, $\sigma = 0.01$
% \label{subfig:sublabel3}
}[ 0.231\textwidth ]
{\includegraphics[width=0.23\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_2_nrR_10/f1_Gaussian_f_sigma_0p01_k_3_lambda_0p3_scanID_2_nrReps_10.eps} }
\hspace{0.01\textwidth} % seperation
%------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------
%
%
%
\subcaptionbox[]{ $k=2$, $\lambda= 0.1$, $\sigma = 0.05$
% \label{subfig:sublabel3}
}[ 0.231\textwidth ]
{\includegraphics[width=0.23\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_2_nrR_10/f1_Gaussian_f_sigma_0p05_k_2_lambda_0p1_scanID_2_nrReps_10.eps} }
\hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{ $k=3$, $\lambda= 0.1$, $\sigma = 0.05$
% \label{subfig:sublabel3}
}[ 0.231\textwidth ]
{\includegraphics[width=0.23\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_2_nrR_10/f1_Gaussian_f_sigma_0p05_k_3_lambda_0p1_scanID_2_nrReps_10.eps} }
\hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{ $k=2$, $\lambda= 0.3$, $\sigma = 0.05$
% \label{subfig:sublabel3}
}[ 0.231\textwidth ]
{\includegraphics[width=0.23\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_2_nrR_10/f1_Gaussian_f_sigma_0p05_k_2_lambda_0p3_scanID_2_nrReps_10.eps} }
\hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{ $k=3$, $\lambda= 0.3$, $\sigma = 0.05$
% \label{subfig:sublabel3}
}[ 0.231\textwidth ]
{\includegraphics[width=0.23\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_2_nrR_10/f1_Gaussian_f_sigma_0p05_k_3_lambda_0p3_scanID_2_nrReps_10.eps} }
\hspace{0.01\textwidth} % seperation
%------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------
%
\subcaptionbox[]{ $k=2$, $\lambda= 0.1$, $\sigma = 0.15$
% \label{subfig:sublabel3}
}[ 0.231\textwidth ]
{\includegraphics[width=0.23\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_2_nrR_10/f1_Gaussian_f_sigma_0p15_k_2_lambda_0p1_scanID_2_nrReps_10.eps} }
\hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{ $k=3$, $\lambda= 0.1$, $\sigma = 0.15$
% \label{subfig:sublabel3}
}[ 0.231\textwidth ]
{\includegraphics[width=0.23\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_2_nrR_10/f1_Gaussian_f_sigma_0p15_k_3_lambda_0p1_scanID_2_nrReps_10.eps} }
\hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{ $k=2$, $\lambda= 0.3$, $\sigma = 0.15$
% \label{subfig:sublabel3}
}[ 0.231\textwidth ]
{\includegraphics[width=0.23\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_2_nrR_10/f1_Gaussian_f_sigma_0p15_k_2_lambda_0p3_scanID_2_nrReps_10.eps} }
\hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{ $k=3$, $\lambda= 0.3$, $\sigma = 0.15$
% \label{subfig:sublabel3}
}[ 0.231\textwidth ]
{\includegraphics[width=0.23\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_2_nrR_10/f1_Gaussian_f_sigma_0p15_k_3_lambda_0p3_scanID_2_nrReps_10.eps} }
\hspace{0.01\textwidth} % seperation
%------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------
%
%%%%%%
\subcaptionbox[]{ $k=2$, $\lambda= 0.1$, $\sigma = 0.25$
% \label{subfig:sublabel3}
}[ 0.231\textwidth ]
{\includegraphics[width=0.23\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_2_nrR_10/f1_Gaussian_f_sigma_0p25_k_2_lambda_0p1_scanID_2_nrReps_10.eps} }
\hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{ $k=3$, $\lambda= 0.1$, $\sigma = 0.25$
% \label{subfig:sublabel3}
}[ 0.231\textwidth ]
{\includegraphics[width=0.23\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_2_nrR_10/f1_Gaussian_f_sigma_0p25_k_3_lambda_0p1_scanID_2_nrReps_10.eps} }
\hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{ $k=2$, $\lambda= 0.3$, $\sigma = 0.25$
% \label{subfig:sublabel3}
}[ 0.231\textwidth ]
{\includegraphics[width=0.23\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_2_nrR_10/f1_Gaussian_f_sigma_0p25_k_2_lambda_0p3_scanID_2_nrReps_10.eps} }
\hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{ $k=3$, $\lambda= 0.3$, $\sigma = 0.25$
% \label{subfig:sublabel3}
}[ 0.231\textwidth ]
{\includegraphics[width=0.23\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_2_nrR_10/f1_Gaussian_f_sigma_0p25_k_3_lambda_0p3_scanID_2_nrReps_10.eps} }
\hspace{0.01\textwidth} % seperation
%------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------
\vspace{3mm}
\caption[Short Caption]{ f1 Gaussian: f, nrReps = 10, scanID = 2
% Numerical results for the function XYZ, under the Gaussian noise model.  Results are averaged over 20 trials, $n=500, k \in  \{ 2,3,5 \}$ and $\lambda \in \{ 0.1, 0.3, 0.5, 1 \} $  
}
\label{fig:Sims_f1_Gaussian_ScanID2_f}
\end{figure*}
\fi 

==> AISTATS_input_experiments-backup.tex <==


\vspace{-4mm}
%----------------------------------
% Numerical experiments
%----------------------------------
\section{Numerical experiments} \label{sec:num_exps}
\vspace{-3mm}
This section contains numerical experiments for the two noise models 
discussed in Section \ref{sec:ProblemSetup}, namely the Uniform model (with samples generated uniformly in $[-\gamma,\gamma]$ for bounded $\gamma$) 
and Gaussian models. For each experiment, we show the RMSE error on a log scale, for denoised samples of $f \mod 1$ 
and $f$. We compare  the performance of three algorithms. 

%
%\begin{itemize}
%\item 
\textbf{OLS} denotes the algorithm based on the least squares formulation \ref{item:ols_unwrap} used to recover samples of $f$, 
and works directly with noisy $\bmod 1$ samples; the estimated $f \mod 1$ values are then obtained as the corresponding  
$\bmod 1$ versions.
%
%\item 
\textbf{QCQP} denotes Algorithm \ref{algo:two_stage_denoise} where the unwrapping stage is performed via \textbf{OLS} \ref{item:ols_unwrap}.
%
%\item 
\textbf{iQCQP} denotes an iterated version of \textbf{QCQP}, wherein we repeatedly denoise
the noisy $f \mod 1$ estimates (via Stage $1$ of Algorithm \ref{algo:two_stage_denoise}) for $l$ iterations, 
and finally perform the unwrapping stage via \textbf{OLS} \ref{item:ols_unwrap}, to recover the sample estimates of $f$.
%\end{itemize}
%
%
In other words, all three methods recover the final sample estimates of $f$ via the least squares formulation \ref{item:ols_unwrap}, 
the difference being that \textbf{OLS}  takes as input the initially given noisy $f \mod 1$ samples, while \textbf{QCQP} 
and \textbf{iQCQP} first denoise the $f \mod 1$ samples. 
%
% 
\iffalse
\begin{figure*}
\centering
\subcaptionbox[]{  $\sigma=0.1$
% \label{subfig:sublabel3}
}[ 0.3\textwidth ]
{\includegraphics[width=0.29\textwidth] {figs/delta_corrs/f1_Gaussian_sigma_0p1_n_500_delta_y_vs_delta_l.eps} }
\hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{  $\sigma=0.1$,
% \label{subfig:sublabel3}
}[ 0.67\textwidth ]
{\includegraphics[width=0.67\textwidth] {figs/delta_corrs/f1_Gaussian_sigma_0p1_n_500_fmod1CleanNoise.eps} }
\hspace{0.01\textwidth} % seperation
% 
%
\subcaptionbox[]{  $\sigma=0.15$
% \label{subfig:sublabel3}
}[ 0.3\textwidth ]
{\includegraphics[width=0.29\textwidth] {figs/delta_corrs/f1_Gaussian_sigma_0p15_n_500_delta_y_vs_delta_l.eps} }
\hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{  $\sigma=0.15$,
% \label{subfig:sublabel3}
}[ 0.67\textwidth ]
{\includegraphics[width=0.67\textwidth] {figs/delta_corrs/f1_Gaussian_sigma_0p15_n_500_fmod1CleanNoise.eps} }
\hspace{0.01\textwidth} % seperation
% 
%
\subcaptionbox[]{  $\sigma=0.2$
% \label{subfig:sublabel3}
}[ 0.3\textwidth ]
{\includegraphics[width=0.29\textwidth] {figs/delta_corrs/f1_Gaussian_sigma_0p2_n_500_delta_y_vs_delta_l.eps} }
\hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{  $\sigma=0.2$,
% \label{subfig:sublabel3}
}[ 0.67\textwidth ]
{\includegraphics[width=0.67\textwidth] {figs/delta_corrs/f1_Gaussian_sigma_0p2_n_500_fmod1CleanNoise.eps} }
% \hspace{0.01\textwidth} % seperation
% 
\vspace{-2mm}
\caption[Short Caption]{ f1 Gaussian: instance, $n=500$. Left: scatter plot of change in $y$ (the observed noisy mode 1 values) versus change in $l$ (the noisy quotient). Right: plot of the clean f mod 1 values (red), and the noisy f mod 1 values (blue).
}
\label{fig:instances_f1_Gaussian_delta_cors}
\end{figure*}
\fi
%
%
%    
Figure \ref{fig:instances_f1_Bounded} shows several denoising instances as we increase the noise level 
in the Uniform noise model, $\gamma \in \{0.15, 0.27, 0.30\}$, to illustrate the decay in performance of 
\textbf{OLS}, \textbf{QCQP}, and \textbf{iQCQP} ($10$ iterations). 
%Figure \ref{fig:instances_f1_Gaussian} shows analogous results for the Gaussian model, 
%with $\sigma \in \{0.05, 0.13, 0.17\}$.
Analogous results for the Gaussian model are shown in the appendix.
%
%
%
\begin{figure*}
\centering
\subcaptionbox[]{  $\gamma=0.15$, \textbf{OLS}
% \label{subfig:sublabel3}
}[ 0.26\textwidth ]
{\includegraphics[width=0.20\textwidth] {figs/instances/f1_Bounded_sigma_0p15_n_500_k_2_lambda_0p1_instance_OLS.eps} }
% \hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{  $\gamma=0.15$, \textbf{QCQP}
% \label{subfig:sublabel3}
}[ 0.26\textwidth ]
{\includegraphics[width=0.20\textwidth] {figs/instances/f1_Bounded_sigma_0p15_n_500_k_2_lambda_0p1_instance_QCQP.eps} }
% \hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{  $\gamma=0.15$, \textbf{iQCQP}  (10  iters.)
% \label{subfig:sublabel3}
}[ 0.26\textwidth ]
{\includegraphics[width=0.20\textwidth] {figs/instances/f1_Bounded_sigma_0p15_n_500_k_2_lambda_0p1_instance_iQCQP.eps} }
% \hspace{0.01\textwidth} % seperation
%
% 
% \newline

\subcaptionbox[]{  $\gamma=0.27$, \textbf{OLS}
% \label{subfig:sublabel3}
}[ 0.26\textwidth ]
{\includegraphics[width=0.20\textwidth] {figs/instances/f1_Bounded_sigma_0p27_n_500_k_2_lambda_0p1_instance_OLS.eps} }
% \hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{  $\gamma=0.27$, \textbf{QCQP}
% \label{subfig:sublabel3}
}[ 0.26\textwidth ]
{\includegraphics[width=0.20\textwidth] {figs/instances/f1_Bounded_sigma_0p27_n_500_k_2_lambda_0p1_instance_QCQP.eps} }
% \hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{  $\gamma=0.27$, \textbf{iQCQP} (10 iters.)
% \label{subfig:sublabel3}
}[ 0.26\textwidth ]
{\includegraphics[width=0.20\textwidth] {figs/instances/f1_Bounded_sigma_0p27_n_500_k_2_lambda_0p1_instance_iQCQP.eps} }
% \hspace{0.01\textwidth} % seperation
%
% 
% \newline

\subcaptionbox[]{  $\gamma=0.30$, \textbf{OLS}
% \label{subfig:sublabel3}
}[ 0.26\textwidth ]
{\includegraphics[width=0.20\textwidth] {figs/instances/f1_Bounded_sigma_0p3_n_500_k_2_lambda_0p1_instance_OLS.eps} }
% \hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{  $\gamma=0.30$, \textbf{QCQP}
% \label{subfig:sublabel3}
}[ 0.26\textwidth ]
{\includegraphics[width=0.20\textwidth] {figs/instances/f1_Bounded_sigma_0p3_n_500_k_2_lambda_0p1_instance_QCQP.eps} }
% \hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{  $\gamma=0.30$, \textbf{iQCQP}  (10 iters.)
% \label{subfig:sublabel3}
}[ 0.26\textwidth ]
{\includegraphics[width=0.20\textwidth] {figs/instances/f1_Bounded_sigma_0p3_n_500_k_2_lambda_0p1_instance_iQCQP.eps} }
% \hspace{0.01\textwidth} % seperation
%
% 
%
% \newline
\iffalse
\subcaptionbox[]{  $\gamma=0.34$, \textbf{OLS}
% \label{subfig:sublabel3}
}[ 0.26\textwidth ]
{\includegraphics[width=0.20\textwidth] {figs/instances/f1_Bounded_sigma_0p34_n_500_k_2_lambda_0p1_instance_OLS.eps} }
% \hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{  $\gamma=0.34$, \textbf{QCQP}
% \label{subfig:sublabel3}
}[ 0.26\textwidth ]
{\includegraphics[width=0.20\textwidth] {figs/instances/f1_Bounded_sigma_0p34_n_500_k_2_lambda_0p1_instance_QCQP.eps} }
% \hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{  $\gamma=0.34$, \textbf{iQCQP} (10 iters.)
% \label{subfig:sublabel3}
}[ 0.26\textwidth ]
{\includegraphics[width=0.20\textwidth] {figs/instances/f1_Bounded_sigma_0p34_n_500_k_2_lambda_0p1_instance_iQCQP.eps} }
% \hspace{0.01\textwidth} % seperation
\fi 
%
% 
\vspace{-2mm}
\caption[Short Caption]{Denoised instances under the Uniform noise model, for \textbf{OLS}, \textbf{QCQP} and \textbf{iQCQP},  as we increase the noise level $\gamma$. We keep fixed the parameters $n=500$, $k=2$, $\lambda= 0.1$.
% Numerical results for the function XYZ, under the Gaussian noise model.  Results are averaged over 20 trials, $n=500, k \in  \{ 2,3,5 \}$ and $\lambda \in \{ 0.1, 0.3, 0.5, 1 \} $  
}
\label{fig:instances_f1_Bounded}
\end{figure*}


%
%
%
% \input{AISTATS_figures_ScanID_1}
%
In Figures \ref{fig:Sims_f1_Bounded_fmod1}, \ref{fig:Sims_f1_Bounded_f}, we assess the robustness of the three algorithms 
for the Uniform noise model, and show the RMSE (on a log scale) for denoising $f \mod 1$ and $f$ samples, over different 
noise levels, with $k \in \{2,3\}$ and $\lambda \in \{0.3, 0.5\}$.
%
\begin{figure*}
\centering
\subcaptionbox[]{ $k=2$, $\lambda= 0.03$
% \label{subfig:sublabel3}
}[ 0.24\textwidth ]
{\includegraphics[width=0.24\textwidth] {figs/PLOTS_SCANS/f1_Bounded_scanID_1_nrR_20/f1_Bounded_fmod1_n_500_k_2_lambda_0p03_scanID_1_nrReps_20.eps} }
% \hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{ $k=3$, $\lambda= 0.03$
% \label{subfig:sublabel3}
}[ 0.24\textwidth ]
{\includegraphics[width=0.24\textwidth] {figs/PLOTS_SCANS/f1_Bounded_scanID_1_nrR_20/f1_Bounded_fmod1_n_500_k_3_lambda_0p03_scanID_1_nrReps_20.eps} }
% \hspace{0.01\textwidth} % seperation
%------------------------------------------------------------------------------------------
\subcaptionbox[]{ $k=2$, $\lambda= 0.3$
% \label{subfig:sublabel3}
}[ 0.24\textwidth ]
{\includegraphics[width=0.24\textwidth] {figs/PLOTS_SCANS/f1_Bounded_scanID_1_nrR_20/f1_Bounded_fmod1_n_500_k_2_lambda_0p3_scanID_1_nrReps_20.eps} }
% \hspace{0.01\textwidth} % seperation
%------------------------------------------------------------------------------------------
\subcaptionbox[]{ $k=2$, $\lambda= 0.5$
% \label{subfig:sublabel3}
}[ 0.24\textwidth ]
{\includegraphics[width=0.24\textwidth] {figs/PLOTS_SCANS/f1_Bounded_scanID_1_nrR_20/f1_Bounded_fmod1_n_500_k_2_lambda_0p5_scanID_1_nrReps_20.eps} }
% \hspace{0.01\textwidth} % seperation
%
%------------------------------------------------------------------------------------------
\vspace{-3mm}
\caption[Short Caption]{Numerical experiments of \textbf{OLS}, \textbf{QCQP}, and  \textbf{iQCQP} (with 3,5, and 10 iterations) showing the recovery RMSE error (on a log scale) when denoising the $f \mod 1$ samples, under the Uniform noise model. Results are averaged over 20 trials.
%  f1 Bounded: f mod 1, nrReps = 20, scanID = 1 
% Numerical results for the function XYZ, under the Gaussian noise model.  Results are averaged over 20 trials, $n=500, k \in  \{ 2,3,5 \}$ and $\lambda \in \{ 0.1, 0.3, 0.5, 1 \} $  
}
\label{fig:Sims_f1_Bounded_fmod1}
\end{figure*}
%
%
%
%
%
\begin{figure*}
\centering
\subcaptionbox[]{ $k=2$, $\lambda= 0.03$
% \label{subfig:sublabel3}
}[ 0.24\textwidth ]
{\includegraphics[width=0.24\textwidth] {figs/PLOTS_SCANS/f1_Bounded_scanID_1_nrR_20/f1_Bounded_f_n_500_k_2_lambda_0p03_scanID_1_nrReps_20.eps} }
% \hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{ $k=3$, $\lambda= 0.03$
% \label{subfig:sublabel3}
}[ 0.24\textwidth ]
{\includegraphics[width=0.24\textwidth] {figs/PLOTS_SCANS/f1_Bounded_scanID_1_nrR_20/f1_Bounded_f_n_500_k_3_lambda_0p03_scanID_1_nrReps_20.eps} }
\hspace{0.01\textwidth} % seperation
%
%------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------
%
\subcaptionbox[]{ $k=2$, $\lambda= 0.3$
% \label{subfig:sublabel3}
}[ 0.24\textwidth ]
{\includegraphics[width=0.24\textwidth] {figs/PLOTS_SCANS/f1_Bounded_scanID_1_nrR_20/f1_Bounded_f_n_500_k_2_lambda_0p3_scanID_1_nrReps_20.eps} }
% \hspace{0.01\textwidth} % seperation
%
%------------------------------------------------------------------------------------------
\subcaptionbox[]{ $k=2$, $\lambda= 0.5$
% \label{subfig:sublabel3}
}[ 0.24\textwidth ]
{\includegraphics[width=0.24\textwidth] {figs/PLOTS_SCANS/f1_Bounded_scanID_1_nrR_20/f1_Bounded_f_n_500_k_2_lambda_0p5_scanID_1_nrReps_20.eps} }
% \hspace{0.01\textwidth} % seperation
%
%------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------
\vspace{-3mm}
\caption[Short Caption]{Recovery errors for the final estimate of $f$, under the Uniform noise model (20 trials).
% Numerical experiments showing the recovery error for the final estimate of $f$, under the Uniform noise model   (20 trials). % . Results are averaged over 20 experiments.
%  f1 Bounded: f, nrReps = 20, scanID = 1 
% Numerical results for the function XYZ, under the Gaussian noise model.  Results are averaged over 20 trials, $n=500, k \in  \{ 2,3,5 \}$ and $\lambda \in \{ 0.1, 0.3, 0.5, 1 \} $  
}
\label{fig:Sims_f1_Bounded_f}
\end{figure*}
%
%
%
%
%
Figures \ref{fig:Sims_f1_Gaussian_fmod1}, \ref{fig:Sims_f1_Gaussian_f} show similar plots for the Gaussian noise model.


\begin{figure*}
\centering
\subcaptionbox[]{ $k=2$, $\lambda= 0.1$
% \label{subfig:sublabel3}
}[ 0.24\textwidth ]
{\includegraphics[width=0.24\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_1_nrR_20/f1_Gaussian_fmod1_n_500_k_2_lambda_0p1_scanID_1_nrReps_20.eps} }
%\hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{ $k=3$, $\lambda= 0.1$
% \label{subfig:sublabel3}
}[ 0.24\textwidth ]
{\includegraphics[width=0.24\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_1_nrR_20/f1_Gaussian_fmod1_n_500_k_3_lambda_0p1_scanID_1_nrReps_20.eps} }
% \hspace{0.01\textwidth} % seperation
%------------------------------------------------------------------------------------------
%
\subcaptionbox[]{ $k=2$, $\lambda= 0.3$
% \label{subfig:sublabel3}
}[ 0.24\textwidth ]
{\includegraphics[width=0.24\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_1_nrR_20/f1_Gaussian_fmod1_n_500_k_2_lambda_0p3_scanID_1_nrReps_20.eps} }
%\hspace{0.01\textwidth} % seperation
%------------------------------------------------------------------------------------------
%
\subcaptionbox[]{$k=2$, $\lambda= 0.5$
% \label{subfig:sublabel3}
}[ 0.24\textwidth]
{\includegraphics[width=0.24\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_1_nrR_20/f1_Gaussian_fmod1_n_500_k_2_lambda_0p5_scanID_1_nrReps_20.eps} }
%\hspace{0.01\textwidth} % seperation
%------------------------------------------------------------------------------------------
\vspace{-3mm}
\caption[Short Caption]{Recovery errors for the denoised $f$ \hspace{-2mm} $\mod 1$ samples, for the Gaussian noise model (20 trials). % Results are averaged over 20 runs.
% f1 Gaussian: f mod 1, nrReps = 20, scanID = 1 
% Numerical results for the function XYZ, under the Gaussian noise model.  Results are averaged over 20 trials, $n=500, k \in  \{ 2,3,5 \}$ and $\lambda \in \{ 0.1, 0.3, 0.5, 1 \} $  
}
\label{fig:Sims_f1_Gaussian_fmod1}
\end{figure*}
%----------------------------
 

%-----------------------------
\begin{figure*}
\centering
\subcaptionbox[]{ $k=2$, $\lambda= 0.1$
% \label{subfig:sublabel3}
}[ 0.24\textwidth ]
{\includegraphics[width=0.24\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_1_nrR_20/f1_Gaussian_f_n_500_k_2_lambda_0p1_scanID_1_nrReps_20.eps} }
%\hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{ $k=3$, $\lambda= 0.1$
% \label{subfig:sublabel3}
}[ 0.24\textwidth ]
{\includegraphics[width=0.24\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_1_nrR_20/f1_Gaussian_f_n_500_k_3_lambda_0p1_scanID_1_nrReps_20.eps} }
%\hspace{0.01\textwidth} % seperation
%------------------------------------------------------------------------------------------
\subcaptionbox[]{ $k=2$, $\lambda= 0.3$
% \label{subfig:sublabel3}
}[ 0.24\textwidth ]
{\includegraphics[width=0.24\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_1_nrR_20/f1_Gaussian_f_n_500_k_2_lambda_0p3_scanID_1_nrReps_20.eps} }
% \hspace{0.01\textwidth} % seperation
%------------------------------------------------------------------------------------------
\subcaptionbox[]{ $k=2$, $\lambda= 0.5$
% \label{subfig:sublabel3}
}[ 0.24\textwidth ]
{\includegraphics[width=0.24\textwidth] {figs/PLOTS_SCANS/f1_Gaussian_scanID_1_nrR_20/f1_Gaussian_f_n_500_k_2_lambda_0p5_scanID_1_nrReps_20.eps} }
% \hspace{0.01\textwidth} % seperation
%------------------------------------------------------------------------------------------
\vspace{-3mm}
\caption[Short Caption]{Recovery errors for the final estimated $f$, under the Gaussian noise model (20 trials). % Results are averaged over 20 runs.
%  f1 Gaussian: f, nrReps = 20, scanID = 1 
% Numerical results for the function XYZ, under the Gaussian noise model.  Results are averaged over 20 trials, $n=500, k \in  \{ 2,3,5 \}$ and $\lambda \in \{ 0.1, 0.3, 0.5, 1 \} $  
}
\label{fig:Sims_f1_Gaussian_f}
\end{figure*}
%
% \input{AISTATS_figures_ScanID_2}
%
%
% Figure \ref{fig:Sims_f1_Bounded_ScanID2_fmod1}, respectively Figure \ref{fig:Sims_f1_Bounded_ScanID2_f},
Figure \ref{fig:Sims_f1_Bounded_ScanID2_ffmod1} shows the RMSE (on a log scale) for the denoised $f \mod 1$ 
samples (leftmost two plots) and samples of $f$ (rightmost two plots), as a function of $n$. 
This is shown for $\lambda=0.3$, $k \in \{ 2,3 \}$ and $\gamma \in \{0.01, 0.25\}$ for the Uniform noise model.
%
%

\begin{figure*}
\centering
%%%%
\subcaptionbox[]{ $k=2$, $\lambda= 0.3$, $\gamma = 0.01$
% \label{subfig:sublabel3}
}[ 0.24\textwidth ]
{\includegraphics[width=0.24\textwidth] {figs/PLOTS_SCANS/f1_Bounded_scanID_2_nrR_10/f1_Bounded_fmod1_sigma_0p01_k_2_lambda_0p3_scanID_2_nrReps_10.eps} }
% \hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{ $k=3$, $\lambda= 0.3$, $\gamma = 0.25$
% \label{subfig:sublabel3}
}[ 0.24\textwidth ]
{\includegraphics[width=0.24\textwidth] {figs/PLOTS_SCANS/f1_Bounded_scanID_2_nrR_10/f1_Bounded_fmod1_sigma_0p25_k_3_lambda_0p3_scanID_2_nrReps_10.eps} }
% \hspace{0.01\textwidth} % seperation
%------------------------------------------------------------------------------------------
%
% \iffalse
% ------------------------------------------------------------------------------------------
%\vspace{-3mm}
%\caption[Short Caption]{ f1 Bounded: f mod 1, nrReps = 10, scanID = 2
% Numerical results for the function XYZ, under the Gaussian noise model.  Results are averaged over 20 trials, $n=500, k \in  \{ 2,3,5 \}$ and $\lambda \in \{ 0.1, 0.3, 0.5, 1 \} $  
%}
%\label{fig:Sims_f1_Bounded_ScanID2_fmod1}
%\end{figure}
%\begin{figure}
% \centering
% \fi  
%
\subcaptionbox[]{ $k=2$, $\lambda= 0.3$, $\delta = 0.01$
% \label{subfig:sublabel3}
}[ 0.24\textwidth ]
{\includegraphics[width=0.24\textwidth] {figs/PLOTS_SCANS/f1_Bounded_scanID_2_nrR_10/f1_Bounded_f_sigma_0p01_k_2_lambda_0p3_scanID_2_nrReps_10.eps} }
% \hspace{0.01\textwidth} % seperation
%
\subcaptionbox[]{ $k=3$, $\lambda= 0.3$, $\delta = 0.25$
% \label{subfig:sublabel3}
}[ 0.24\textwidth ]
{\includegraphics[width=0.24\textwidth] {figs/PLOTS_SCANS/f1_Bounded_scanID_2_nrR_10/f1_Bounded_f_sigma_0p25_k_3_lambda_0p3_scanID_2_nrReps_10.eps} }
% \hspace{0.01\textwidth} % sepe, ration
%------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------
\vspace{-3mm}
\caption[Short Caption]{Recovery errors for \textbf{OLS}, \textbf{QCQP}, and  \textbf{iQCQP} 
% (with 3,5, and 10 iterations) 
as a function of $n$ (number of samples), for both the $f \mod 1$ samples (leftmost two plots) and the final $f$ estimates (rightmost two plots) under the Uniform noise model, for different values of $k$, $\lambda$ and $\delta$. Results are averaged over 20 runs.
% f1 Bounded: f, nrReps = 10, scanID = 2
% Numerical results for the function XYZ, under the Gaussian noise model.  Results are averaged over 20 trials, $n=500, k \in  \{ 2,3,5 \}$ and $\lambda \in \{ 0.1, 0.3, 0.5, 1 \} $  
}
% \label{fig:Sims_f1_Bounded_ScanID2_f}
\label{fig:Sims_f1_Bounded_ScanID2_ffmod1}
\end{figure*}

%We refer the reader to the Appendix for an extensive set of numerical results that extend those 
%illustrated in Figures \ref{fig:Sims_f1_Bounded_fmod1} (Uniform, $f \mod 1$) \ref{fig:Sims_f1_Bounded_f} (Uniform, $f$), 
%\ref{fig:Sims_f1_Gaussian_fmod1} (Gaussian, $f \mod 1$), \ref{fig:Sims_f1_Gaussian_f} (Gaussian, $f$), where we 
%vary $k \in \{2,3,5 \}$ and $\lambda \in \{0.1, 0.3, 0.5, 1 \}$, to show the interplay between these parameters.


==> AISTATS_preamble_labels.tex <==
% \usepackage[margin=1in]{geometry}

%%% \usepackage[top=24mm, bottom=18mm, left=15mm, right=13mm,headsep=0.5 cm,footnotesep=0.2cm]{geometry}
 
% LOUT: AISTAST 
% \usepackage[top=12mm, left=10mm, right=40mm]{geometry}
 
\usepackage[]{amsmath,amssymb,epsfig}
% \usepackage{subfigure}
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{comment}
\usepackage{array}
\usepackage{algorithm}
\usepackage{url}

\usepackage{lscape}
\usepackage{algpseudocode}
\usepackage{setspace}
\usepackage{multicol}
\usepackage{multirow}
\usepackage{color}
\usepackage{colortbl}
\usepackage{xcolor}
\usepackage{hyperref}

\usepackage[%
    font={small,sf},
    labelfont=bf,
    format=hang,    
    format=plain,
    margin=0pt,
    width=0.8\textwidth,
]{caption}
\usepackage[list=true]{subcaption}



%-----------------------------
% Theorem like environments
%-----------------------------
\newtheorem{theorem}{Theorem}
% \theoremstyle{plain}
\newtheorem{acknowledgment}{Acknowledgment}
\newtheorem{assumption}{Assumption}
\newtheorem{axiom}{Axiom}
\newtheorem{case}{Case}
\newtheorem{claim}{Claim}
\newtheorem{conclusion}{Conclusion}
\newtheorem{condition}{Condition}
\newtheorem{conjecture}{Conjecture}
\newtheorem{corollary}{Corollary}
\newtheorem{criterion}{Criterion}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{exercise}{Exercise}
\newtheorem{lemma}{Lemma}
\newtheorem{notation}{Notation}
\newtheorem{problem}{Problem}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{solution}{Solution}
\newtheorem{summary}{Summary}
\numberwithin{equation}{section}
%\newtheorem{proof}{Proof}

\newenvironment{rcases}
  {\left.\begin{aligned}}
  {\end{aligned}\right\rbrace}

%---------------------------------------------
% Commands for symbols used in the report.
% \mathcal symbols
%----------------------------------------------
\newcommand{\calA}{\ensuremath{\mathcal{A}}}
\newcommand{\calB}{\ensuremath{\mathcal{B}}}
\newcommand{\calC}{\ensuremath{\mathcal{C}}}
\newcommand{\calD}{\ensuremath{\mathcal{D}}}
\newcommand{\calH}{\ensuremath{\mathcal{H}}}
\newcommand{\calF}{\ensuremath{\mathcal{F}}}
\newcommand{\calG}{\ensuremath{\mathcal{G}}}
\newcommand{\calI}{\ensuremath{\mathcal{I}}}
\newcommand{\calP}{\ensuremath{\mathcal{P}}}
\newcommand{\calPp}{\ensuremath{\calP^{\prime}}}
\newcommand{\calR}{\ensuremath{\mathcal{R}}}
\newcommand{\calS}{\ensuremath{\mathcal{S}}}
\newcommand{\calM}{\ensuremath{\mathcal{M}}}
\newcommand{\calN}{\ensuremath{\mathcal{N}}}
\newcommand{\calT}{\ensuremath{\mathcal{T}}}
\newcommand{\calU}{\ensuremath{\mathcal{U}}}
\newcommand{\calK}{\ensuremath{\mathcal{K}}}
\newcommand{\calX}{\ensuremath{\mathcal{X}}}
\newcommand{\calV}{\ensuremath{\mathcal{V}}}
\newcommand{\calY}{\ensuremath{\mathcal{Y}}}
\newcommand{\calE}{\ensuremath{\mathcal{E}}}

% Miscellaneous symbols 
\newcommand{\tri}{\ensuremath{\bigtriangleup}}
\newcommand{\norm}[1]{\parallel{#1}\parallel}
\newcommand{\abs}[1]{|{#1}|}
\newcommand{\ceil}[1]{\lceil{#1}\rceil}
\newcommand{\floor}[1]{\lfloor{#1}\rfloor}
\newcommand{\set}[1]{\left\{{#1}\right\}}
\newcommand{\dotprod}[2]{\langle#1,#2\rangle}
\newcommand{\est}[1]{\widehat{#1}}
\newcommand{\expec}{\ensuremath{\mathbb{E}}}
\newcommand{\matR}{\ensuremath{\mathbb{R}}}
\newcommand{\matZ}{\ensuremath{\mathbb{Z}}}
\newcommand{\argmax}[1]{\underset{#1}{\operatorname{argmax}}}
\newcommand{\argmin}[1]{\underset{#1}{\operatorname{argmin}}}
\newcommand{\ubar}[1]{\underaccent{\bar}{#1}}
\newcommand{\prob}{\ensuremath{\mathbb{P}}}
\newcommand{\Linfnorm}{L_{\infty}}
\newcommand{\todo}[1]{\textbf{TODO: #1}}

%Indicator variable
\newcommand{\indic}{\ensuremath{\mathbbm{1}}} 

% Vectors and matrices
\newcommand{\vecx}{\mathbf x}
\newcommand{\vecn}{\mathbf n}
\newcommand{\vecp}{\mathbf p}
\newcommand{\vecq}{\mathbf q}
\newcommand{\veci}{\mathbf i}
\newcommand{\vecj}{\mathbf j}
\newcommand{\vecu}{\mathbf u}
\newcommand{\vecv}{\mathbf v}
\newcommand{\vecw}{\mathbf w}
\newcommand{\vecb}{\mathbf b}
\newcommand{\vecm}{\mathbf m}
\newcommand{\vecc}{\mathbf c}
\newcommand{\vecy}{\mathbf y}
\newcommand{\vecf}{\mathbf f}
\newcommand{\vecz}{\mathbf z}
\newcommand{\veca}{\mathbf a}
\newcommand{\vecg}{\mathbf g}
\newcommand{\veco}{\mathbf 0}
\newcommand{\matA}{\ensuremath{\mathbf{A}}}
\newcommand{\matB}{\ensuremath{\mathbf{B}}}
\newcommand{\matI}{\ensuremath{\mathbf{I}}}
\newcommand{\matV}{\ensuremath{\mathbf{V}}}
\newcommand{\matH}{\ensuremath{\mathbf{H}}}
\newcommand{\matX}{\ensuremath{\mathbf{X}}}
\newcommand{\matP}{\ensuremath{\mathbf{P}}}

\newcommand{\real}{\text{Re}}
\newcommand{\imag}{\text{Im}}
\newcommand{\vecgbar}{\bar{\mathbf g}}
\newcommand{\vecgbarest}{\est{\vecgbar}}
%\newcommand{\Hbar}{\bar{H}}
\newcommand{\Hbar}{H}
\newcommand{\veczbar}{\bar{\mathbf z}}

%---- Added by HT on 10th Oct ----------------
\newcommand{\vecgest}{\est{\vecg}}
\newcommand{\gest}{\est{g}}
\newcommand{\qtathresh}{\zeta}
\newcommand{\sign}{\text{sign}}
%--------------------------------------------
%\newcommand{\gtil}{\tilde{g}}
%\newcommand{\gtilbar}{\bar{\tilde{g}}}
%\newcommand{\vecgtil}{\mathbf{\tilde{g}}}
%\newcommand{\vecgtilbar}{\mathbf{\bar{\tilde{g}}}}

% leave out.. make sure code does not crash...
% \newcommand{\gtil}{h}
% \newcommand{\gtilbar}{\bar{h}}
% \newcommand{\vecgtil}{\mathbf{h}}
% \newcommand{\vecgtilbar}{\bar{\mathbf{h}}}

\newcommand{\htil}{h}
\newcommand{\htilbar}{\bar{h}}
\newcommand{\vechtil}{\mathbf{h}}
\newcommand{\vechtilbar}{\bar{\mathbf{h}}}

% replaced    \gtil by  \htil  						in all 5 files 
% replace      \gtilbar by   \htilbar    (never used actually ... )
% replaced    \vecgtil  by   \vechtil     		in all 5 files 
% replaced \vecgtilbar   by \vechtilbar 		 in all 5 files 

\newcommand{\mean}{{\bar{\boldsymbol{\mu}}}}

\newcommand{\trseq}{\ensuremath{TSR_{=}}}
\newcommand{\trsineq}{\ensuremath{TSR_{\leq}}}
 
  
\usepackage{rotating}
%\usepackage[right]{showlabels}
%\renewcommand{\showlabelsetlabel}[1]
%{\begin{turn}{0}\showlabelfont #1\end{turn}}
    
\newcommand{\vecdelta}{\boldsymbol{\delta}}
    
\newcommand{\mb}[1]{\mbox{\boldmath$#1$}}
   
   
